Cascaded Cross-Attention Networks for Data-Efficient Whole-Slide Image Classification Using Transformers

Whole-Slide Imaging allows for the capturing and digitization of high-resolution images of histological specimen. An automated analysis of such images using deep learning models is therefore of high demand. The transformer architecture has been proposed as a possible candidate for effectively leveraging the high-resolution information. Here, the whole-slide image is partitioned into smaller image patches and feature tokens are extracted from these image patches. However, while the conventional transformer allows for a simultaneous processing of a large set of input tokens, the computational demand scales quadratically with the number of input tokens and thus quadratically with the number of image patches. To address this problem we propose a novel cascaded cross-attention network (CCAN) based on the cross-attention mechanism that scales linearly with the number of extracted patches. Our experiments demonstrate that this architecture is at least on-par with and even outperforms other attention-based state-of-the-art methods on two public datasets: On the use-case of lung cancer (TCGA NSCLC) our model reaches a mean area under the receiver operating characteristic (AUC) of 0.970 $\pm$ 0.008 and on renal cancer (TCGA RCC) reaches a mean AUC of 0.985 $\pm$ 0.004. Furthermore, we show that our proposed model is efficient in low-data regimes, making it a promising approach for analyzing whole-slide images in resource-limited settings. To foster research in this direction, we make our code publicly available on GitHub: XXX.

==> backup.tex <==
\subsection{WSI classification}
We compare the performance of the models on two publicly available datasets, comprising cancer subtype classification tasks (TCGA NSCLC and TCGA RCC) and cancer detection (CAMELYON16). For the binary classification tasks (i.e., tumor vs no tumor in CAMELYON16 and LUSC vs LUAD in TCGA NSCLC), we use the area under the receiver operating characteristic (AUC), to assess the model performance. For the multiclass classification problems (i.e., KICH vs KIRC vs KIRP in TCGA RCC), we assess the performance by computing the (macro-averaged) one vs. rest AUC. To guarantee a fair comparison, we train all models on the exact same data splits of the 4-fold cross validation. For TCGA NSCLC, we find that our model outperforms the TransMIL baseline (AUC: 0.970 vs 0.957) and thereby sets a new state of the art for the TCGA NSCLC subtype classification task. Similarly, we find that on the TCGA RCC dataset our model is on par with the state-of-the-art results set by TransMIL (both reach an AUC of 0.985, see Figure \ref{results} for a more detailed comparison). 
